Toward Real-World Super-Resolution via Adaptive Downsampling Models

Most image super-resolution (SR) methods are developed on synthetic low-resolution (LR) and high-resolution (HR) image pairs that are constructed by a predetermined operation, e.g., bicubic downsampling. As existing methods typically learn an inverse mapping of the specific function, they produce blurry results when applied to real-world images whose exact formulation is different and unknown. Therefore, several methods attempt to synthesize much more diverse LR samples or learn a realistic downsampling model. However, due to restrictive assumptions on the downsampling process, they are still biased and less generalizable. This study proposes a novel method to simulate an unknown downsampling process without imposing restrictive prior knowledge. We propose a generalizable low-frequency loss (LFL) in the adversarial training framework to imitate the distribution of target LR images without using any paired examples. Furthermore, we design an adaptive data loss (ADL) for the downsampler, which can be adaptively learned and updated from the data during the training loops. Extensive experiments validate that our downsampling model can facilitate existing SR methods to perform more accurate reconstructions on various synthetic and real-world examples than the conventional approaches.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/1_intro.tex <==
\ifCLASSOPTIONcompsoc
\IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
\else
\section{Introduction}
\label{sec:introduction}
\fi

\IEEEPARstart{I}{mage} super-resolution (SR), which aims to reconstruct a high-resolution~(HR) image from a low-resolution~(LR) input, plays an essential role in computer vision and digital photography.
%
There exist numerous applications, including enhancing the details and photorealism of an image~\cite{sr_srgan}, high-quality editing~\cite{sr_explorable}, and breaking the sensor limitation of mobile cameras~\cite{wronski2019handheld}.
%
Recently, a plethora of SR methods have been developed on the basis of deep CNNs~\cite{sr_srcnn, sr_lapsrn, sr_srgan, sr_edsr} and large-scale datasets~\cite{data_div2k, sr_edsr}.
%
However, state-of-the-art methods~\cite{sr_esrgan, sr_rcan, sr_dbpn, sr_rdn} do not generalize well to the real-world inputs even they perform relatively well on synthesized, e.g., bicubic-downsampled, LR images.
%
In overcoming this issue, few recent approaches~\cite{sr_zllz, sr_camera, sr_realworld, sr_cdc} have collected high-quality pairs of real-world LR and HR examples to learn their SR models.
%
Nevertheless, such an acquisition process remains to be challenging due to outdoor scene dynamics and spatial misalignments~\cite{sr_zllz}.


Conventional SR methods synthesize various LR samples $\img{LR}$ from ground-truth HR images $\img{HR}$ by the following:
%
\begin{equation}
    \img{LR} = \paren{ \img{HR} \ast k }_{\downarrow s} + n,
    \label{eq:linear}
\end{equation}
%
where $k \in \mathbb{R}^{2}$ is a 2D degradation kernel, $\ast$ is a spatial convolution, $_{\downarrow s}$ is a decimation with a stride $s$, and $n$ is a noise term.
%
The decimation operator corresponds to direct downsampling mentioned in the super-resolution literature~\cite{sr_srmd}.
%
With a specific assumption of blur kernels, e.g., variants of Gaussian~\cite{sr_ikc, sr_blindsr, sr_srmd}, LR and HR pairs can be synthesized to train the following SR models.
%
However, such prior typically limit the kernel space, and the synthesized LR images may not reflect the distribution of real-world inputs~\cite{sr_camera}.
%
Therefore, the learned SR models become less generalizable toward arbitrary real-world input images.

\input{sections/figure/teaser}

On the other hand, recent unsupervised methods simulate real-world LR samples that contain unknown noise~\cite{sr_deg, sr_unpaired_pesudo} and artifacts~\cite{sr_unsupervised, sr_gandeg}.
%
Without using a paired dataset, they first learn a downsampling model under adversarial training frameworks~\cite{gans} to imitate the distribution of real-world images.
%
The following SR models can then be trained in a supervised manner on the simulated dataset to deliver accurate reconstruction results on the real-world inputs.
%
One of the challenges in such methods arises from preserving image content across different scales, i.e., HR and LR, while learning the downsampling model.
%
Existing approaches deal with this problem using a predetermined downsampling operator, e.g., bicubic downsampling, in their objective functions and constrain the simulated LR images not to deviate much from the known formulations.
%
However, the manual selection of the operator can introduce a bias in the unsupervised learning framework, which can also act as a restrictive prior if the ground-truth downsampling model is much different from the used one.
%
%In particular, the learned downsampling model can be biased toward the selected operator rather than being used to simulate the desired distribution of LR images.
%
While KernelGAN~\cite{sr_kernelgan} alleviates the issue by estimating a low-dimensional downsampling kernel $k$ in \eqref{eq:linear} from an LR image $\img{LR}$, various regularization terms need to be applied to restrict the diversity of the possible kernel space.


Therefore, we propose an effective way of imitating the real-world LR samples of an unknown distribution to address the aforementioned issues.
%
Similar to the previous unsupervised methods~\cite{sr_unsupervised, sr_kernelgan}, we also train a downsampling CNN to simulate the LR images in our target distribution.
%
However, rather than formulating the objective function with a handcrafted downsampling operator, we propose a novel and generalizable low-frequency loss (LFL) that does not pose substantial bias.
%
Our LFL facilitates the downsampling model to learn much more diverse and precise functions without being constrained to a specific prior assumption.
%
Furthermore, we develop an adaptive data loss (ADL) that iteratively adjusts the training objective for the given dataset and stabilizes the learning process.
%
As shown in Fig.~\ref{fig:teaser}, our unsupervised learning framework is straightforward, effective, and generalizable to arbitrary downsampling models.
%
Extensive experiments validate that the SR models learned on our downsampled images perform favorably on synthetic and real-world LR images.
%
The contributions of this study can be organized threefold:
%
\begin{compactitem}[$\bullet$]
\item We present a novel unsupervised learning framework to learn an unknown downsampling process without using any HR and LR image pairs.
%
\item We propose LFL and ADL to simulate accurate and realistic LR samples from HR images without relying on any predetermined downsampling operators.
%
\item We demonstrate that the proposed method can be easily integrated with existing SR frameworks and achieve much better results on synthetic and real-world images.
%
\end{compactitem}

==> sections/figure/teaser.tex <==
\begin{figure}
    \vspace{-7mm}
    \centering
    \subfigure[Bicubic]{\includegraphics[width=0.19\linewidth]{figs/teaser/1_bic.png}}
    %
    \subfigure[\cite{sr_esrgan}]{\includegraphics[width=0.19\linewidth]{figs/teaser/1_rrdb.png}}
    %
    \subfigure[\cite{sr_kernelgan} + \cite{sr_zssr}]{\includegraphics[width=0.19\linewidth]{figs/teaser/1_kernelgan.png}}
    %
    \subfigure[\textbf{Ours}]{\includegraphics[width=0.19\linewidth]{figs/teaser/1_akl.png}}
    %
    \subfigure[GT]{\includegraphics[width=0.19\linewidth]{figs/teaser/1_hr.png}}
    \figspace
    %
    \caption{
        \textbf{$\times 4$ SR results on a real-world LR image.}
        %
        (a) LR image magnified with bicubic interpolation.
        %
        (b) Result of RRDB~\cite{sr_esrgan}.
        %
        (c) Result of KernelGAN~\cite{sr_kernelgan} + ZSSR~\cite{sr_zssr}.
        %
        (d) Our unsupervised approach (ADL + RRDB) reconstructs a sharp and visually pleasing output without artifacts and aliasing compared with the existing methods.
        %
        (e) Ground-truth patch from RealSR-V3~\cite{sr_realworld}.
        %
        Images are cropped from `\emph{Canon/045.png}.'
    }
    \label{fig:teaser}
    \figxspace
\end{figure}
